Probabilistic Parking Functions

We consider the notion of classical parking functions by introducing randomness and a new parking protocol, as inspired by the work presented in the paper ``Parking Functions: Choose your own adventure,'' (arXiv:2001.04817) by Carlson, Christensen, Harris, Jones, and Rodr\'iguez. Among our results, we prove that the probability of obtaining a parking function, from a length $n$ preference vector, is independent of the probabilistic parameter $p$. We also explore the properties of a preference vector given that it is a parking function and discuss the effect of the probabilistic parameter $p$. Of special interest is when $p=1/2$, where we demonstrate a sharp transition in some parking statistics. We also present several interesting combinatorial consequences of the parking protocol. In particular, we provide a combinatorial interpretation for the array described in OEIS A220884 as the expected number of preference sequences with a particular property related to occupied parking spots, which solves an open problem of Novelli and Thibon posed in 2020 (arXiv:1209.5959). Lastly, we connect our results to other weighted phenomena in combinatorics and provide further directions for research.

==> table3wayoneway.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
\hline
$\textbf{(1,1,1)}$ & $\textbf{(1,1,2)}$ & $\textbf{(1,1,3)}$ & $\textbf{(1,2,3)}$ & $\textbf{(1,3,2)}$ & $\textbf{(1,2,1)}$ & $\textbf{(1,3,1)}$ & $\textbf{(1,2,2)}$ & $(1,3,3)$  \\ 
\hline
$(2,2,2)$ & $\textbf{(2,2,1)}$ & $(2,2,3)$ & $\textbf{(2,1,3)}$ & $\textbf{(2,3,1)}$ & $\textbf{(2,1,2)}$ & $(2,3,2)$ & $\textbf{(2,1,1)}$ & $(2,3,3)$  \\ 
\hline
$(3,3,3)$ & $(3,3,1)$ & $(3,3,2)$ & $\textbf{(3,2,1)}$ & $\textbf{(3,1,2)}$ & $(3,1,3)$ & $(3,2,3)$ & $\textbf{(3,1,1)}$ & $(3,2,2)$  \\
\hline
\end{tabular}

